SAN: Structure-Aware Network for Complex and Long-tailed Chinese Text Recognition

In text recognition, complex glyphs and tail classes have always been factors affecting model performance. Specifically for Chinese text recognition, the lack of shape-awareness can lead to confusion among close complex characters. Since such characters are often tail classes that appear less frequently in the training-set, making it harder for the model to capture its shape information. Hence in this work, we propose a structure-aware network utilizing the hierarchical composition information to improve the recognition performance of complex characters. Implementation-wise, we first propose an auxiliary radical branch and integrate it into the base recognition network as a regularization term, which distills hierarchical composition information into the feature extractor. A Tree-Similarity-based weighting mechanism is then proposed to further utilize the depth information in the hierarchical representation. Experiments demonstrate that the proposed approach can significantly improve the performances of complex characters and tail characters, yielding a better overall performance. Code is available at https://github.com/Levi-ZJY/SAN.

==> experiments.tex <==
\section{Experiment}

\subsection{Implementation Details}
The datasets used in our experiments are Web Dataset and Scene Dataset~\cite{fudanvi}. The Web Dataset contains 20000 Chinese and English web text images from 17 different categories on the Taobao website and the Scene Dataset contains 636455 text images from several competitions, papers, and projects.

We implement our method with PyTorch and conduct experiments on three NVIDIA RTX 3060 GPUs. 
Each input Image is resized to $32\times128$ with data augmentation.
The batch size is set to 96 and ADAM optimizer is adopted with the initial learning rate $1e^{-4}$, which is decayed to $1e^{-5}$ after 12 epochs.



\subsection{Ablative Study}
\begin{table}[t]
    \caption{Ablation study of ARB. The dataset used is Web dataset~\cite{fudanvi}}

    \centering
    \begin{tabular}{|c|c|c||c|c|}
        \hline
         Model& Naive Radical loss & TreeSim weighing loss & Accuracy & 1-NED \\
         \hline
         VM-Base& & & 59.1 & 0.768 \\
         VM-Naive& \checkmark & & 60.7 & 0.779 \\
         \textbf{VM-TreeSim} & \checkmark &\checkmark& \textbf{61.3} & \textbf{0.786} \\
         \hline
         ABINet-Base & & & 65.6 & 0.803  \\
         ABINet-Naive &\checkmark & & 66.8 & 0.812  \\
         \textbf{ABINet-TreeSim (SAN)}  &\checkmark &\checkmark & \textbf{67.3} & \textbf{0.817} \\
         \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}

We discuss the performance of the proposed approaches~(ARB and TreeSim weighting) with two base-model configurations: Vision Model and ABINet. Experiment results are recorded in Tab.1. From the statistics we can conclude:
1)The proposed ARB is useful, which enhances the accuracy in both VM and ABINet. VM-Naive outperforms VM-Base by 1.6$\%$ accuracy and 0.011 1-NED, ABINet-Naive outperforms ABINet-Base by 1.2$\%$ accuracy and 0.009 1-NED. 
2)TreeSim enhanced weighting achieved the expected results. VM-TreeSim boosts accuracy by 0.6$\%$ and  1-NED by 0.007 than VM-Naive, SAN boosts accuracy by 0.5$\%$ and 1-NED by 0.005 than ABINet-Naive.

The above observations suggest that the hierarchical components information is useful to the feature extractor, which can significantly improve the performance of the vision model. The proposed approaches also yields significant improvement against full ABINet indicating hierarchical components information is still plays a significant part, even when the language models can   








\subsection{Comparative Experiments}
%1) compare with sota(fudanvi).

\begin{table}[t]
    \caption{Performance on Chinese text recognition benchmarks~\cite{fudanvi}. $\dagger$ indicates results reported by ~\cite{fudanvi}, $*$ indicates results from our experiments. }

    \centering
    \begin{tabular}{|c||c|c|c|c|}
        \hline
         Method & \multicolumn{2}{c|}{Web} & \multicolumn{2}{c|}{Scene}  \\
         \hhline{~----}
         & Accuracy  &1-NED &Accuracy&1-NED\\
         \hline
         CRNN$\dagger$~\cite{CRNN} & 54.5&0.736 & 53.4&0.734   \\
         ASTER$\dagger$~\cite{ASTER} & 52.3&0.689 & 54.5&0.695  \\
         MORAN$\dagger$~\cite{moran} & 49.9&0.682 & 51.8&0.686  \\
         SAR$\dagger$~\cite{SAR} & 54.3&0.725 & 62.5&0.785 \\
         SRN$\dagger$~\cite{SRN} & 52.3&0.706 & 60.1&0.778   \\
         SEED$\dagger$~\cite{seed} & 46.3&0.637 & 49.6&0.661  \\
         TransOCR$\dagger$~\cite{Chen2021SceneTT} & 62.3&0.787 & 63.3&0.802 \\
         TransOCR-PRAB$\dagger$~\cite{fudanvi} & 63.8&0.794 & 71.0 &0.843 \\ 
         ABINet$*$~\cite{ABINet} & 65.6 & 0.803 & 71.8 & 0.853 \\
         \hline
         SAN (Ours) & \textbf{67.3} & \textbf{0.817} & \textbf{73.6} & \textbf{0.863} \\
         \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}


Compared with Chinese text recognition benchmarks and recent SOTA works that are trained on web and scene datasets, ARB also shows impressive performance(Tab.2). We can see from the comparison, our SAN outperforms ABINet with 1.7$\%$, 1.8$\%$ on Web and Scene datasets respectively. Also, SAN achieves the best 1-NED on both datasets. Some successful recognition examples are shown in Fig.4, which shows the complex characters and long-tailed characters that predict failure using the base model (ABINet) while predicted successfully by the full model.



\begin{figure}[t]	
\centering
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/comp1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/comp2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/tail1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{Successful recognition examples using ARB. (a) (b) are complex character examples. (c) (d) are long-tailed character examples. Text strings are ABINet prediction, SAN prediction and Ground Trues.}
\end{figure}
\begin{figure}[t]	
\centering
    \subfigure[Web Dataest]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=4cm,width=5.4cm]{figures/amount-web-RSSL.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.9cm,width=5.4cm]{figures/amount-scene-RSSL.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{The ratio of both correct characters and either wrong characters(SAN\ding{51} ABI\ding{55}, SAN\ding{55} ABI\ding{51} and both wrong) divided by RSSL.}
%\vspace{-3mm}
\end{figure}
\subsection{Property analysis}
%The improvements on the TED (the bars you made a few weeks ago.)



To validate the optimization of ARB on complex character recognition and long-tailed character recognition, we divide them into different groups according to their complexity and frequency. For each category, the differences in recognizing performances are first analyzed. 
To give a better understanding of the performance differences, the misrecognized characters by at least one model (misrecognized by SAN, ABINet, or both) are studied in more detail.
Specifically, the average TreeSim between the ground-truth and predicted characters are computed as a rough indicator of structural information awareness.

%To validate the optimization of ARB on complex character recognition and long-tailed character recognition,
%we select the misrecognized characters of SAN and ABINet, divide them into different groups according to their complexity and frequency, and investigate the difference on average TreeSim.

%To validate the optimization of ARB on complex character recognition and long-tailed character recognition, we select the both misrecognized characters of ARB-TreeSim and ABINet, divide them into different groups according to their complexity and frequency, and investigate the difference on average TreeSim.

\subsubsection{Experiments on different complexity characters}







\begin{figure}[t]	
\centering
    \subfigure[Web Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-web1.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-web2.png}%{figures/web-radicalLen2-complex.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-scene1.png}%{figures/scene-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-scene2.png}%{figures/scene-radicalLen2-complex.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
\caption{Average TreeSim divided by RSSL on samples at least misrecognized by one model. RSSL is the length of the radical structure sequence of a character.}
%\vspace{-3mm}
\end{figure}


We observe that the complexity of the character structure is proportional to its radical structure sequence length~(RSSL), so we use RSSL to represent the complexity of the character. 
We select the complex characters, whose RSSL is equal to or longer than 5, and divide them into three parts: 5$\leq{}$RSSL$\leq{}$6~(average 37$\%$ in web and 37$\%$ in scene), RSSL=7~(average 16$\%$ in web and 18$\%$ in scene), RSSL$\ge$8~(average 12$\%$ in web and 14$\%$ in scene).
The ratio of both correct characters and either wrong characters in these three parts are in Fig.5. 
The results suggest that complex characters indeed cause recognition problems, as the more complex the characters are, the less accurate the models get. 
Also, the results suggest the proposed SAN always gets higher accuracy on complex character recognition than the base model(ABINet).


%We observe that the complexity of the character structure is proportional to its radical structure sequence length(RSSL), so we use RSSL to represent the complexity of the character. 
%Besides, we notice that most RSSL is equal to 3, 5, and 7.
%We also notice that the complexity of RSSL5(characters that RSSL is equal to five) is medium, characters with longer RSSL are often complex and characters with shorter RSSL are simple. 
%At the same time, these three parts also have a similar quantity of characters.
%Hence we use RSSL5 as the dividing line and divide misrecognized characters into three parts: RSSL below five(average 35$\%$ in web and 31$\%$ in scene), RSSL equal to five(average 35$\%$ in web and 35$\%$ in scene) and RSSL above five(average 30$\%$ in web and 34$\%$ in scene), which we call them simple characters, sub-complex characters, and complex characters.



We calculate the average TreeSim between either wrong characters and ground trues in these three parts~(Fig.6).
From the result, we can see in web dataset~(Fig.6 (a)) that although the average TreeSim of 5$\leq{}$RSSL$\leq{}$6 characters decreases slightly, both the RSSL=7 characters and the RSSL$\ge{}$8 characters are increasing, and the rise of RSSL$\ge{}$8 characters are extremely significant.
In scene dataset~(Fig.6 (b)), the average TreeSim of the three parts are all increasing, and the rise of 5$\leq{}$RSSL$\leq{}$6 and RSSL=7 characters are both obvious.
The experiment shows that ARB can prominently improve the similarity between the recognition results and ground trues of complex characters, indicating that ARB has a more distinct perception of complex characters, 
which is due to the introduction of hierarchical structure information improving the \textawareness{} of the vision model and making it easier for models to distinguish different components in complex characters.


%We calculate the average TreeSim between misrecognized characters and ground trues in these three parts(Fig.6).
%From the result, we can see in web dataset, the average TreeSim of complex characters decreases most obviously. 
%In scene dataset, the average TreeSim of sub-complex characters decreases most obviously and complex characters also have a large decrease.
%The experiment shows that ARB can prominently improve the similarity between the recognition results and ground trues of complex characters, indicating that ARB has a more distinct perception of complex characters, 
%which is due to the introduction of hierarchical structure information improving the \textawareness{} of the vision model and making it easier for models to distinguish different components in complex characters.



\subsubsection{Experiments on long-tailed characters}


\begin{figure}[h]	
\centering
    \subfigure[Web Dataest]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.7cm,width=5cm]{figures/amount-web-OccN.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.7cm,width=5cm]{figures/amount-scene-OccN.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{The ratio of both correct characters and either wrong characters(SAN\ding{51} ABI\ding{55}, SAN\ding{55} ABI\ding{51} and both wrong) divided by OccN.}
\label{fig:occnchar}
%\vspace{-3mm}
\end{figure}


\begin{figure}[htbp]	
\centering
    \subfigure[Web Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-web1.png}%{figures/web-frequency1-tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-web2.png}%{figures/web-frequency2-tail2.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-scene1.png}%{figures/scene-frequency1-tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-scene2.png}%{figures/scene-frequency2-tail2.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
\caption{Average TreeSim divided by OccN on samples at least misrecognized by one model. OccN is the occurrence number of a character in the training dataset. }
%\vspace{-3mm}
\end{figure}


To validate the optimation of our model on long-tailed characters, we sort misrecognized characters in descending according to their occurrence number in the training dataset, select the characters whose occurrence number is less than 100, and divide them into three parts: 100$>$OccN$\ge$50~(average 9$\%$ in web and 11$\%$ in scene), 50$>$OccN$\ge$20~(average 11$\%$ in web and 15$\%$ in scene), 20$>$OccN$\ge$0~(average 16$\%$ in web and 27$\%$ in scene).
The ratio of both correct characters and either wrong characters in these three parts are in Fig.~\ref{fig:occnchar}.
Results indicate that data sufficiency is a more significant problem than structural complexity, where the proposed SAN is significantly less affected compared to the base model. However, the results also indicate that the proposed methods do not fully solve all the problems caused by tail classes, which remain to be a future topic.
 

%To validate the optimation on long-tailed characters, we sort both misrecognized characters in descending according to their occurrence number in the training dataset, then divide them into four parts according to their frequency. The first part is the characters in the first 25$\%$ of the frequency, which is called head classes, and the last part is the characters in the last 25$\%$ of the frequency, which is called tail classes.


We calculate the average TreeSim between either wrong characters and ground trues in these parts~(Fig.8).
The result shows that there is obviously increasing in average TreeSim on tail classes. 
%In web dataset, we can see the decline trend is increasing when the occurrence number decrease and the average TreeSim of $20>OccN\ge0$ characters decrease most obviously.
In web dataset~(Fig.8 (a)), we can see the TreeSim of 100$>$OccN$\ge{}$50 and 20$>$OccN$\ge{}$0 characters increase obviously.
In scene dataset~(Fig.8 (b)), the average TreeSim of the three parts all has significant increases. The average rise of scene dataset is more than twice of the web dataset.
This result shows that the recognition results of ARB in long-tailed characters are more similar to the ground trues, 
indicating that ARB can learn more features of long-tailed characters,
which is because of the common components combination traits shared between characters, ARB can take advantage of the traits learning on head classes to optimize the tail classes recognition.

%We calculate the average TreeSim between misrecognized characters and ground trues in these parts(Fig.7).
%The result shows that there are obviously decreasing in average TreeSim on tail classes, and the decline is significantly higher than other parts in both web and scene dataset.
%This result indicates that ARB has significant improvement in the recognition of long-tailed characters, which is because of the common components combination traits shared between characters, ARB can take advantage of the traits learning on head classes to optimize the tail classes recognition.








==> experiments_change.tex <==
\section{Experiment}

\subsection{Implementation Details}
The datasets used in our experiments are Web Dataset and Scene Dataset~\cite{fudanvi}. The Web Dataset contains 20000 Chinese and English web text images from 17 different categories on the Taobao website and the Scene Dataset contains 636455 text images from several competitions, papers, and projects.

We implement our method with PyTorch and conduct experiments on three NVIDIA RTX 3060 GPUs. 
Each input Image is resized to $32\times128$ with data augmentation.
The batch size is set to 96 and ADAM optimizer is adopted with the initial learning rate $1e^{-4}$, which is decayed to $1e^{-5}$ after 12 epochs.



\subsection{Ablative Study}
\begin{table}[t]
    \caption{Ablation study of ARB. The dataset used is Web dataset~\cite{fudanvi}}

    \centering
    \begin{tabular}{|c|c|c||c|c|}
        \hline
         Model& Naive Radical loss & TreeSim weighing loss & Accuracy & 1-NED \\
         \hline
         VM-Base& & & 59.1 & 0.768 \\
         VM-Naive& \checkmark & & 60.7 & 0.779 \\
         \textbf{VM-TreeSim} & \checkmark &\checkmark& \textbf{61.3} & \textbf{0.786} \\
         \hline
         ABINet-Base & & & 65.6 & 0.803  \\
         ABINet-Naive &\checkmark & & 66.8 & 0.812  \\
         \textbf{ABINet-TreeSim (SAN)}  &\checkmark &\checkmark & \textbf{67.3} & \textbf{0.817} \\
         \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}

We discuss the performance of the proposed approaches~(ARB and TreeSim weighting) with two base-model configurations: Vision Model and ABINet. Experiment results are recorded in Tab.1. From the statistics we can conclude:
1)The proposed ARB is useful, which enhances the accuracy in both VM and ABINet. VM-Naive outperforms VM-Base by 1.6$\%$ accuracy and 0.011 1-NED, ABINet-Naive outperforms ABINet-Base by 1.2$\%$ accuracy and 0.009 1-NED. 
2)TreeSim enhanced weighting achieved the expected results. VM-TreeSim boosts accuracy by 0.6$\%$ and  1-NED by 0.007 than VM-Naive, SAN boosts accuracy by 0.5$\%$ and 1-NED by 0.005 than ABINet-Naive.

The above observations suggest that the hierarchical components information is useful to the feature extractor, which can significantly improve the performance of the vision model. The proposed approaches also yields significant improvement against full ABINet indicating hierarchical components information is still plays a significant part, even when the language models can   








\subsection{Comparative Experiments}
%1) compare with sota(fudanvi).

\begin{table}[t]
    \caption{Performance on Chinese text recognition benchmarks~\cite{fudanvi}. $\dagger$ indicates results reported by ~\cite{fudanvi}, $*$ indicates results from our experiments. }

    \centering
    \begin{tabular}{|c||c|c|c|c|}
        \hline
         Method & \multicolumn{2}{c|}{Web} & \multicolumn{2}{c|}{Scene}  \\
         \hhline{~----}
         & Accuracy  &1-NED &Accuracy&1-NED\\
         \hline
         CRNN$\dagger$~\cite{CRNN} & 54.5&0.736 & 53.4&0.734   \\
         ASTER$\dagger$~\cite{ASTER} & 52.3&0.689 & 54.5&0.695  \\
         MORAN$\dagger$~\cite{moran} & 49.9&0.682 & 51.8&0.686  \\
         SAR$\dagger$~\cite{SAR} & 54.3&0.725 & 62.5&0.785 \\
         SRN$\dagger$~\cite{SRN} & 52.3&0.706 & 60.1&0.778   \\
         SEED$\dagger$~\cite{seed} & 46.3&0.637 & 49.6&0.661  \\
         TransOCR$\dagger$~\cite{Chen2021SceneTT} & 62.3&0.787 & 63.3&0.802 \\
         TransOCR-PRAB$\dagger$~\cite{fudanvi} & 63.8&0.794 & 71.0 &0.843 \\ 
         ABINet$*$~\cite{ABINet} & 65.6 & 0.803 & 71.8 & 0.853 \\
         \hline
         SAN (Ours) & \textbf{67.3} & \textbf{0.817} & \textbf{73.6} & \textbf{0.863} \\
         \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}


Compared with Chinese text recognition benchmarks and recent SOTA works that are trained on web and scene datasets, ARB also shows impressive performance(Tab.2). We can see from the comparison, our SAN outperforms ABINet with 1.7$\%$, 1.8$\%$ on Web and Scene datasets respectively. Also, SAN achieves the best 1-NED on both datasets. Some successful recognition examples are shown in Fig.4, which shows the complex characters and long-tailed characters that predict failure using the base model (ABINet) while predicted successfully by the full model.



\begin{figure}[t]	
\centering
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/comp1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/comp2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/tail1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2.2cm,width=3cm]{figures/tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{Successful recognition examples using ARB. (a) (b) are complex character examples. (c) (d) are long-tailed character examples. Text strings are ABINet prediction, SAN prediction and Ground Trues.}
\end{figure}
\begin{figure}[t]	
\centering
    \subfigure[Web Dataest]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=4cm,width=5.4cm]{figures/amount-web-RSSL.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.9cm,width=5.4cm]{figures/amount-scene-RSSL.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{The ratio of both correct characters and either wrong characters(SAN\ding{51} ABI\ding{55}, SAN\ding{55} ABI\ding{51} and both wrong) divided by RSSL.}
%\vspace{-3mm}
\end{figure}
\subsection{Property analysis}
%The improvements on the TED (the bars you made a few weeks ago.)



To validate the effectiveness of ARB on complex character recognition and long-tailed character recognition, we divide them into different groups according to their complexity and frequency. For each category, the differences in recognizing performances are first analyzed. 
To give a better understanding of the performance differences, the misrecognized characters by at least one model (misrecognized by SAN, ABINet, or both) are studied in more detail.
Specifically, the average TreeSim between the ground-truth and predicted characters are computed as a rough indicator of structural information awareness.

%To validate the optimization of ARB on complex character recognition and long-tailed character recognition,
%we select the misrecognized characters of SAN and ABINet, divide them into different groups according to their complexity and frequency, and investigate the difference on average TreeSim.

%To validate the optimization of ARB on complex character recognition and long-tailed character recognition, we select the both misrecognized characters of ARB-TreeSim and ABINet, divide them into different groups according to their complexity and frequency, and investigate the difference on average TreeSim.

\subsubsection{Experiments on different complexity characters}







\begin{figure}[t]	
\centering
    \subfigure[Web Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-change-web1.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-change-web2.png}%{figures/web-radicalLen2-complex.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-change-scene1.png}%{figures/scene-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/RSSL-change-scene2.png}%{figures/scene-radicalLen2-complex.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
\caption{Average TreeSim divided by RSSL on samples at least misrecognized by one model. RSSL is the length of the radical structure sequence of a character.}
%\vspace{-3mm}
\end{figure}


We observe that the complexity of the character structure is proportional to its radical structure sequence length~(RSSL), so we use RSSL to represent the complexity of the character. 
We select the complex characters, whose RSSL is equal to or longer than 5, and divide them into three parts: 5$\leq{}$RSSL$\leq{}$6~(average 37$\%$ in web and 37$\%$ in scene), RSSL=7~(average 16$\%$ in web and 18$\%$ in scene), RSSL$\ge$8~(average 12$\%$ in web and 14$\%$ in scene).
The ratio of both correct characters and either wrong characters in these three parts are in Fig.5. 
The results suggest that complex characters indeed cause recognition problems, as the more complex the characters are, the less accurate the models get. 
Also, the results suggest the proposed SAN always gets higher accuracy on complex character recognition than the base model(ABINet).


%We observe that the complexity of the character structure is proportional to its radical structure sequence length(RSSL), so we use RSSL to represent the complexity of the character. 
%Besides, we notice that most RSSL is equal to 3, 5, and 7.
%We also notice that the complexity of RSSL5(characters that RSSL is equal to five) is medium, characters with longer RSSL are often complex and characters with shorter RSSL are simple. 
%At the same time, these three parts also have a similar quantity of characters.
%Hence we use RSSL5 as the dividing line and divide misrecognized characters into three parts: RSSL below five(average 35$\%$ in web and 31$\%$ in scene), RSSL equal to five(average 35$\%$ in web and 35$\%$ in scene) and RSSL above five(average 30$\%$ in web and 34$\%$ in scene), which we call them simple characters, sub-complex characters, and complex characters.



We calculate the average TreeSim between either wrong characters and ground trues in these three parts~(Fig.6).
From the result, we can see in web dataset~(Fig.6 (a)) that although the average TreeSim of 5$\leq{}$RSSL$\leq{}$6 characters decreases slightly, both the RSSL=7 characters and the RSSL$\ge{}$8 characters are increasing, and the rise of RSSL$\ge{}$8 characters are extremely significant.
In scene dataset~(Fig.6 (b)), the average TreeSim of the three parts are all increasing, and the rise of 5$\leq{}$RSSL$\leq{}$6 and RSSL=7 characters are both obvious.
The experiment shows that ARB can prominently improve the similarity between the recognition results and ground trues of complex characters, indicating that ARB has a more distinct perception of complex characters, 
which is due to the introduction of hierarchical structure information improving the \textawareness{} of the vision model and making it easier for models to distinguish different components in complex characters.


%We calculate the average TreeSim between misrecognized characters and ground trues in these three parts(Fig.6).
%From the result, we can see in web dataset, the average TreeSim of complex characters decreases most obviously. 
%In scene dataset, the average TreeSim of sub-complex characters decreases most obviously and complex characters also have a large decrease.
%The experiment shows that ARB can prominently improve the similarity between the recognition results and ground trues of complex characters, indicating that ARB has a more distinct perception of complex characters, 
%which is due to the introduction of hierarchical structure information improving the \textawareness{} of the vision model and making it easier for models to distinguish different components in complex characters.



\subsubsection{Experiments on long-tailed characters}


\begin{figure}[h]	
\centering
    \subfigure[Web Dataest]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.7cm,width=5cm]{figures/amount-change-OccN-web.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            %\centering          %子图居中
            \includegraphics[height=3.7cm,width=5cm]{figures/amount-change-OccN-scene.png}%{figures/web-radicalLen1-complex.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{The ratio of both correct characters and either wrong characters(SAN\ding{51} ABI\ding{55}, SAN\ding{55} ABI\ding{51} and both wrong) divided by OccN.}
\label{fig:occnchar}
%\vspace{-3mm}
\end{figure}


\begin{figure}[htbp]	
\centering
    \subfigure[Web Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-change-web1.png}%{figures/web-frequency1-tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-change-web2.png}%{figures/web-frequency2-tail2.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
    \subfigure[Scene Dataset]
    {
        \begin{minipage}[t]{0.4\linewidth}
            \centering          %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-change-scene1.png}%{figures/scene-frequency1-tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
        \begin{minipage}[t]{0.4\linewidth}
            \centering      %子图居中
            \includegraphics[height=3.5cm,width=4.7cm]{figures/OccN-change-scene2.png}%{figures/scene-frequency2-tail2.png}
            %\caption{TreeSim Weight}
        \end{minipage}
    }
\caption{Average TreeSim divided by OccN on samples at least misrecognized by one model. OccN is the occurrence number of a character in the training dataset. }
%\vspace{-3mm}
\end{figure}




To validate the optimation of our model on long-tailed characters, we first count the number of character classes in the training dataset where the web training dataset has 4221 classes and the scene training dataset has 5653 classes, and count the occurrence number(OccN) of these classes. Then, we sort character classes in descending according to their OccN, select the last 60$\%$ classes(tail classes) and divide these classes into three parts: last 60$\%$$\sim$last 40$\%$, last 40$\%$$\sim$last 20$\%$ and last 20$\%$$\sim$last 0$\%$. In web, OccN of these three parts are 17$>$OccN$\ge$6, 6$>$OccN$\ge$3 and 3$>$OccN$\ge$0 while in scene are 41$>$OccN$\ge$10, 10$>$OccN$\ge$3 and 3$>$OccN$\ge$0.
The ratio of both correct characters and either wrong characters in these three parts are in Fig.~\ref{fig:occnchar}.
Results indicate that data sufficiency is a more significant problem than structural complexity, where the proposed SAN is significantly less affected compared to the base model. However, the results also indicate that the proposed methods do not fully solve all the problems caused by tail classes, which remain to be a future topic.



%To validate the optimation of our model on long-tailed characters, we sort misrecognized characters in descending according to their occurrence number in the training dataset, select the characters whose occurrence number is less than 100, and divide them into three parts: 100$>$OccN$\ge$50~(average 9$\%$ in web and 11$\%$ in scene), 50$>$OccN$\ge$20~(average 11$\%$ in web and 15$\%$ in scene), 20$>$OccN$\ge$0~(average 16$\%$ in web and 27$\%$ in scene).
%The ratio of both correct characters and either wrong characters in these three parts are in Fig.~\ref{fig:occnchar}.
%Results indicate that data sufficiency is a more significant problem than structural complexity, where the proposed SAN is significantly less affected compared to the base model. However, the results also indicate that the proposed methods do not fully solve all the problems caused by tail classes, which remain to be a future topic.




 We calculate the average TreeSim between either wrong characters and ground trues in these parts~(Fig.8).
%The result shows that there is obviously increasing in average TreeSim on tail classes. 
In web dataset~(Fig.8 (a)),we can see that the average TreeSim of 17$>$OccN$\ge{}$6 characters decreases slightly, the 6$>$OccN$\ge{}$3 characters and the 3$>$OccN$\ge{}$0 characters are increasing, and the rise of 3$>$OccN$\ge{}$0 characters are extremely significant.
In scene dataset~(Fig.8 (b)), the average TreeSim of the three parts are all increasing, and the rise of 3$>$OccN$\ge{}$0 is obvious.
This result shows that the recognition results of ARB in long-tailed characters are more similar to the ground trues, 
indicating that ARB can learn more features of long-tailed characters,
which is because of the common components combination traits shared between characters, ARB can take advantage of the traits learning on head classes to optimize the tail classes recognition.




%We calculate the average TreeSim between either wrong characters and ground trues in these parts~(Fig.8).
%The result shows that there is obviously increasing in average TreeSim on tail classes. 
%%In web dataset, we can see the decline trend is increasing when the occurrence number decrease and the average TreeSim of $20>OccN\ge0$ characters decrease most obviously.
%In web dataset~(Fig.8 (a)), we can see the TreeSim of 100$>$OccN$\ge{}$50 and 20$>$OccN$\ge{}$0 characters increase obviously.
%In scene dataset~(Fig.8 (b)), the average TreeSim of the three parts all has significant increases. The average rise of scene dataset is more than twice of the web dataset.
%This result shows that the recognition results of ARB in long-tailed characters are more similar to the ground trues, 
%indicating that ARB can learn more features of long-tailed characters,
%which is because of the common components combination traits shared between characters, ARB can take advantage of the traits learning on head classes to optimize the tail classes recognition.










==> intro_v1_cat.tex <==
\section{Introduction}
%Part1:
%（why doing this）
Chinese text recognition plays an important role in the field of text recognition due to its huge audience and market. However, the performances of the Chinese text recognition task have often been limited by the large-scale character vocabulary, many complex characters, and the insufficient amount of training samples~\cite{ZeroshotHC}.

%Part2:
%(shortcomings of the existing methods)
Early works in Chinese text recognition are usually character based. Some works are CNN-based  model~\cite{MultiColumnDN,HandwrittenCR,ICDAR2C}. For example, MCDNN~\cite{MultiColumnDN} integrates multiple models including CNN and reaches human-level performance. Wu et al.~\cite{HandwrittenCR} alternatively train a relaxation CNN which regularize the neural network during the training procedure. Later, Du et al.~\cite{DeepNN} attempt to sequentially model the text line and adopt DNN to model the posterior probability of all HMM states. 
In addition, some works pay attention to the characteristics of Chinese text and design targeted optimization strategies~\cite{FromTT,MaximumER,WriterAwareCF,TemplateInstanceLF,JointAA,BuildingFA}. Wu et al~\cite{FromTT} use the MLCA recognition framework and a new writing-style-aware image synthesis method to alleviate the impact caused by the large character set and the lack of training samples.  Wang et al.~\cite{WriterAwareCF} utilize the similarity of Chinese characters to reduce the total number of HMM states. 
%However, all of these methods are based on character, which makes it difficult to further explore the deep features of Chinese characters and solve more complex problems. 
However, the above methods fail to utilize \texthierinfo{} 
of labels~\cite{wubizhengma,taktak,RANRA}, which serves as element-shared and style-invariant descriptors.
This problem makes the aforementioned methods prone to data insufficiency problems in few-shot or zero-shot situations.
 
In this case, several radical-based methods~\cite{RANRA,RadicalAN,ZeroshotHC,DenseRANFO,JointSA} are raised by treating each character as a radical sequence. RAN~\cite{RANRA} employs an attention mechanism to extract radicals from Chinese characters and to detect spatial structures among the radicals. HDE~\cite{ZeroshotHC} designs an embedding vector for each Chinese character, which is based on the radical-level constitution. 
Besides the Chinese language, characters in many other languages can be similarly decomposed into basic components~\cite{taktak,9412607,Rai2021PhoSCNetAA,DBLP:conf/icfhr/ChandaBHHSS18}, where the components and the composition can be hierarchically modeled as a tree, where the basic components serve as leaves and the structural information serves as non-leaf nodes. 

Existing component-based methods demonstrated that structural information helps improve low-shot performance(i.e., the tail classes). In this work, we demonstrate improving structural awareness also alleviates the performance of complex character recognition.
We believe one reason behind the performance issue of complex characters is their complex hierarchical structure which makes it difficult for models to perceive the relationship between components. Since the components and structures are shared among different Chinese characters despite their structural complexity and occurrence frequency, the proposed strategy can improve the recognition performance of both complex characters and the tail classes. 

%bridges common local and structural traits between rare characters and frequent characters.

%（main idea）
%For characters with hierarchical structure~\cite{taktak}, as a tree composed of various components hierarchically, and give the label a hierarchical representation. 
In this work, we choose to validate the aforementioned assumption on the Chinese language, and the hierarchical radical representation~\cite{hde} is adopted to model the structural and component information of each character. 
Based on the radical decomposition method, we propose a strategy to enhance the \textawareness{} of visual features by using the hierarchical representation as a regularization term. 
%Implementation-wise, we adopt the ABINet~\cite{ABINet} as the baseline method. Applying the \textradicalbranch{} yields a novel two branches learning network, which replaces the original Vision Model,  
%where the introduced \textradicalbranch{} acts as a regularization term to distill structural and component information to the shared feature extractor. 
Implementation-wise, we propose a \textradicalbranch{} acts as a regularization term to distill structural and component information into character features, by decoding them into \texthierinfo{}. Not losing generality, we adopt the SOTA ABINet~\cite{ABINet} as the baseline method, and the \textradicalbranch{} is integrated into the Vision model, yielding a novel two branches learning network.
The proposed branch allows the radical level prediction model to supplement and refine the visual feature extraction of the character level prediction model in the training process, which enables the model to focus more on local features and learn more structured visual features.
As basic components are shared among head and tail classes alike, the proposed \textradicalbranch{} also improves the tail-classes performance by explicitly exploiting their connections with head classes.

%In addition, to better evaluate the effect of ARB,
%Based on this, we explore a tree structure information enhancement method for ARB, and further study the role of tree structure information in visual feature extraction.

In addition,   we proposed a novel Tree-Edit Distance method that serves as a more fine-grained metric measuring the visual similarity between two characters.
Based on the new metric, we propose to further exploit the depth information of the hierarchical representation, which is implemented by weighting the tree nodes accordingly in the ARB branch.
Experimental results demonstrate the effectiveness of ARB in optimizing the recognition performance of complex characters and long-tailed characters, and it also improves the overall recognition accuracy of Chinese text.


%（Article Structure）
%Part4:

%（our contribution）
The contributions of this work are as follows:
\begin{itemize}
    \item We propose a new optimization method for complex character recognition by utilizing the radical structure information of character, which also improves the recognition performance of the tail classes.

    \item We propose a novel Tree-Edit Distance method to measure the similarity of two characters, which is hierarchical, bidirectional, and deep-independent.

    \item We propose ARB based on the tree modeling of the label, which enhances the structure awareness of visual features. ARB shows promising improvement in complex character and long-tailed character recognition and it also improves the overall recognition accuracy of Chinese text.


\end{itemize}


==> introv1.tex <==
\section{Introduction}
%Part1:
%（why doing this）
Chinese text recognition plays an important role in the field of text recognition due to its huge audience and market. However, the performance of model in Chinese text has often been limited by the large-scale character vocabulary, many complex characters, and large number of insufficient training samples~\cite{ZeroshotHC}.

%Part2:
%(shortcomings of the existing methods)
Early works in Chinese text recognition are usually character based. Some works are based on CNN model~\cite{MultiColumnDN,HandwrittenCR,ICDAR2C}. For example, MCDNN~\cite{MultiColumnDN} integrates multiple models including CNN and reaches human-level performance. Wu et al.~\cite{HandwrittenCR} alternatively trains a relaxation CNN to regularize the neural network during the training procedure. Later, Du et al.~\cite{DeepNN} attempt to sequentially model the text line and adopt DNN to model the posterior probability of all HMM states. In addition, some works pay attention to the characteristics of Chinese text and design targeted optimization strategies~\cite{FromTT,MaximumER,WriterAwareCF,TemplateInstanceLF,JointAA,BuildingFA}. Wu et al~\cite{FromTT} use MLCA recognition framework and a new writing-style-aware image synthesis method to overcome large character sets and great insufficient training samples problems. Wang et al.~\cite{WriterAwareCF} utilize the similarity of Chinese characters to reduce the total number of HMM states. However, all of these methods are based on character, which makes it difficult to further explore the deep features of Chinese characters and solve more complex problems. In this case, several radical-based methods~\cite{RANRA,RadicalAN,ZeroshotHC,DenseRANFO,JointSA} are raised by treating each character as a radical sequence. RAN~\cite{RANRA} employs an attention mechanism to extract radicals from Chinese characters and to detect spatial structures among the radicals. HDE~\cite{ZeroshotHC} designs an embedding vector for each Chinese character, which is based on the radical-level constitution. However, existing radical-based methods do not deeply explore the role of radical structure information in the optimization of complex character recognition and long-tailed character recognition. 
%At the same time, there is little simple, effective, and universal optimization strategy for these two problems in Chinese text recognition.




%Patr3:
%（motivation）
In this paper, we believe that complex characters are difficult to recognize because of their complex hierarchical structure which makes it difficult for models to perceive the relationship between components.
Hence, we proposed to improve the \textawareness{}, by proposing to exploit the radical information, which models the basic components and the structural information of each character. The basic components and structures are shared among Chinese characters despite their structural complexity and occurrence frequency. 
Hence, we proposed to improve the \textawareness{} by modeling the components and their structural composition of individual characters.
As such traits are commonly shared among frequent (head) and rare (tail) characters, the proposed strategy also improves the recognition performance of the tail classes. 
%bridges common local and structural traits between rare characters and frequent characters.

%（main idea）
%For characters with hierarchical structure~\cite{taktak}, as a tree composed of various components hierarchically, and give the label a hierarchical representation. 
Characters in many languages can be decomposed into basic components~\cite{taktak,9412607,Rai2021PhoSCNetAA,DBLP:conf/icfhr/ChandaBHHSS18}, where the components and the composition can be hierarchically modeled as a tree, where the basic components serve as leaves and the structural information serves as non-leaf nodes. 
In this work, we focus on the Chinese language, and the hierarchical radical representation~\cite{hde} is adopted to model the structural and component information of each character.
Based on this modeling method, we propose a strategy to enhance the \textawareness{} of visual features by using the hierarchical representation as a regularization term. Implementation-wise, we adopt the SOTA ABINet~\cite{ABINet} as the base method to verify the proposed strategy. Applying the \textradicalbranch{} yields a novel two branches learning network, which replaces the original Vision Model,  
where the introduced \textradicalbranch{} acts as a regularization term to distill structural and component information to the shared feature extractor. The proposed branch allows the radical level prediction model to supplement and refine the visual feature extraction of the character level prediction model in the training process, which enables the model to focus more on local features and learn more structured visual features.
As basic components are shared among head and tail classes alike, the proposed \textradicalbranch{} also improves the tail-classes performance by explicitly exploiting their connections with head classes.


In addition, to better evaluate the effect of ARB, we proposed a novel Tree-Edit Distance method to measure the similarity of two characters. Based on this, we explore a tree structure information enhancement method for ARB, and further study the role of tree structure information in visual feature extraction.
Experimental results demonstrate the effectiveness of ARB in optimizing the recognition performance of complex characters and long-tailed characters, and it also improves the overall recognition accuracy of Chinese text.


%（Article Structure）
%Part4:

%（our contribution）
The contributions of this work are as follows:
\begin{itemize}
    \item We propose a new optimization method for complex character recognition by utilizing the radical structure information of character, which also improves the recognition performance of the tail classes.

    \item We proposed a novel Tree-Edit Distance method to measure the similarity of two characters, which is hierarchical, bidirectional, and deep-independent.

    \item We propose ARB based on the tree modeling of the label, which enhances the structure-awareness of visual features. ARB shows promising improvement in complex character and long-tailed character recognition and it also improves the overall recognition accuracy of Chinese text.


\end{itemize}


==> ourmethod_if_cat.tex <==
\section{Our Method}
%\input{ourmethod_intro_v1.tex}
\input{ourmethod_intro_v1_cat.tex}
\begin{figure}[t]	
    \begin{minipage}[t]{0.5\linewidth}
        \centering          %子图居中
        \includegraphics[height=3cm,width=6.2cm]{figures/RadicalTree.png}   
        \caption{Radical Tree. The right side is the result of converting the left radical structure sequence into a tree.}
    \end{minipage}
    \begin{minipage}[t]{0.5\linewidth}
        \centering          %子图居中
    \end{minipage}
    \begin{minipage}[t]{0.5\linewidth}
        \centering          %子图居中
    \end{minipage}
    \begin{minipage}[t]{0.5\linewidth}
        \centering          %子图居中
    \end{minipage}
    \begin{minipage}[t]{0.5\linewidth}
        \centering      %子图居中
        \includegraphics[height=3.5cm,width=4.5cm]{figures/TreeEDWeight.png}
        \caption{TreeED Weight. The yellow circle indicates that the total weight of the subtree is 1/3.}
    \end{minipage}
    \vspace{-7mm}
\end{figure}
\subsection{Label Modeling } 

For character which can be decomposed into basic components, we model it as a tree composed of various components hierarchically, and model the label as a forest composed of character trees, which gives the label a structural representation.
%This representation can improve the \textawareness{} of the vision model and allows it to pay more attention to the details and local features of characters instead of the overall information.

 As shown in Fig.2, in Chinese, one popular modeling method is to decompose characters into radicals and structures~\cite{fudanvi}. 
 Radicals are the basic components of characters, and structures describe the spatial composition of the radicals in each character.
 One structure is often associated with two or more radicals, we can regard it and the associated radicals as a subtree.
 The subtree can be regarded as a big radical, which is connected to another structure to form a larger subtree. 
 In this way, all Chinese characters can be modeled as a tree, in which leaf nodes are radicals, and non-leaf nodes are structures. For simplicity, we call such trees ``radical trees'' in this paper.



\begin{algorithm}[t]\small
    \caption{TreeED Weight Algorithm}  
    \begin{algorithmic}[1]
        %\Require 
        %\Ensure   
        %{\textbf{Input:}}
        \Require  
          $Node$: Pointer of the root node;  
          $W$: Weight of the tree, which is equal to 1;
        \Function {GetTreeEdWeight}{$Node, W$}  
            %\State $n \gets $number of branches of this node  
            \State $n \gets $number of children of this node  
            \If {$n == 0$}  
                \State weight of this node$\gets W$
                \State \Return{}
            \Else
                \State weight of this node$\gets W/(n+1)$
                \For{$c \gets Node.Children$}                    
                    \State \Call{GetTreeEdWeight}{$c, W/(n+1)$}  
                \EndFor
            \EndIf
            \State \Return{}  
        \EndFunction  
    \end{algorithmic}  
\end{algorithm}  

%For two radical trees, which may not be aligned, we want to find a fair and hierarchical method to measure their similarity. 
%Hence, we propose a novel Tree-edit Distance(TreeED).  
%For two radical trees, which may not be aligned, it is necessary to find an appropriate method to measure their similarity. 
%ICDAR 19, ART (1-NED)

In this work, we propose a novel Tree edit Distance(TreeED) metric to 
measure the visual similarity between two characters representated with radical trees.
In a radial tree, the upper components represent large and overall information, while the lower components represent small and local information. When comparing the similarity of two characters, humans tend to pay more attention to the upper components and less attention to the lower ones. 

% \begin{algorithm}[!h]\small
%     \caption{TreeED Weight Algorithm}  
%     \begin{algorithmic}[1]
%         %\Require 
%         %\Ensure   
%         %{\textbf{Input:}}
%         \Require  
%           $Node$: Pointer of the root node;  
%           $W$: Weight of the tree, which is equal to 1;
%         \Function {GetTreeEdWeight}{$Node, W$}  
%             %\State $n \gets $number of branches of this node  
%             \State $n \gets $ degree of this node  
%             \If {$n == 0$}  
%                 \State weight of this node$\gets W$
%                 \State \Return{}
%             \Else
%                 \If {$n == 2$}  
%                     \State weight of this node$\gets W/3$
%                     \State \Call{GetTreeEdWeight}{$Node.leftchild, W/3$}  
%                     \State \Call{GetTreeEdWeight}{$Node.rightchild, W/3$}
%                 \EndIf
%                 \If {$n == 3$}  
%                     \State weight of this node$\gets W/4$
%                     \State \Call{GetTreeEdWeight}{$Node.leftchild, W/4$}
%                     \State \Call{GetTreeEdWeight}{$Node.midchild, W/4$}
%                     \State \Call{GetTreeEdWeight}{$Node.rightchild, W/4$}
%                 \EndIf
%             \EndIf
%             \State \Return{}  
%         \EndFunction  
%     \end{algorithmic}  
% \end{algorithm}  

Correspondingly, as shown in Fig.3, we first propose a weighting method for TreeED. The method includes the following characteristics:
%Correspondingly, Tree-edit Distance includes the following characteristics:
1)Upper components in the radical tree have greater penalty weight. 2)Every subtree is regarded as an independent individual, the root node and its subtrees have equal weight. 3)The total weight of the tree is 1.



%2)The subtree and its root node are considered as a whole, the weight distributed to the root node is distributed to the whole. 3)The total weight of the whole tree is 1, the root node and its directly connected nodes are equally distributed with the root node weight.



%formula
%\begin{equation}
%    w_{leaf} = W_{subtree_i}
%\end{equation}
%\begin{equation}
%    w_{subtree_i-root} = W_{left-subsubtree} = W_{right-subsubtree} = \frac{1}{N}W_{subtree_i}
%\end{equation}
%\begin{equation}
%    W_{subtree_0} = 1
%\end{equation}
%where $W$ is the weight of a whole subtree, $w$ is the weight of a certain node, $N$ is the number of branches of the subtree root, $W_{subtree_0}$ is the whole tree.


Based on this weighting method, the TreeED calculation process is as follows: 1)Select any one of the two radical trees, and traverse every node in preorder.
2)For each node, the matching rules includes: 2.1)Every ancestor of this node is matching. 2.2)This location in the other tree also has a node and the two nodes are the same. 
3)TreeED is equal to the sum of the weights of all matching nodes.

The proposed TreeED is hierarchical, bidirectional, and deep-independent. 
Hierarchical means TreeED pays different attention to different levels of the tree.
Bidirectional means no matter select which of the two trees, the calculation result is the same. 
Depth-independent means the weight of nodes at a certain level is independent of the depth of the tree. 


Based on this label modeling method, we proposed two loss design strategies.
Considering that a rigorous calculation for the loss of two forests may be complex and nonlinear, we introduce two linear approximate calculation methods in 3.2 to supervise the loss calculation.


\begin{figure}[t]	
    \begin{minipage}[b]{1\linewidth}
        \centering         
        \includegraphics[height=6.5cm,width=11cm]{figures/TreeED.png}
        \caption{TreeED calculation. Nodes with a red circle are the match modes and nodes with a black circle are the mismatch nodes. The calculation results of the two radical trees are the same}
    \end{minipage}
    \vspace{-7mm}
\end{figure}


\subsection{Auxiliary Radical Branch} 
As shown in Fig.1.Auxiliary Radical Branch(ARB) includes the following characteristics:1)The label representation in ARB is hierarchical, which contains component and structural information. 2)ARB is regarded as an independent visual perception optimization branch, which takes feature as input, decodes according to structured representation, and finally refine the visual feature extraction.

The role of ARB is reflected in two aspects: One is that ARB can use hierarchical label representation to supply and refine the feature extraction, improving the \textawareness{} of the model.
%push the model to pay more attention to the local features and learn more structured visual representation. 
The other is that by taking advantage of the common component combination traits between Chinese characters, ARB could exploit the component information connections between tail classes and head classes, which can optimize long-tailed character recognition.
%ARB could transfer the learning results from different characters, and optimize the long-tailed character recognition.

In ARB, we propose two linear loss design strategies, which reflect the hierarchical label representation while simplifying the design and calculation.


\subsubsection{Sequence Modeling}

%The Chinese label is hierarchically modeled as a forest (discussed in 3.1), 
Considering that the proposed label modeling method is top-down and root-first, in loss design, we intend to perpetuate this design mode to match them.
We propose using the sequence by traversing the radical tree in preorder to model each tree in the label, so we use the linear radical structure sequence~\cite{fudanvi}.
%We propose to model the label by concatenating the pre-order traverse of the component tree of each character. Implementation-wise,  we adopt the character representation in ~\cite{fudanvi}. 
This sequence follows the root-first design strategy and retains the hierarchical structure information of the radical tree to a certain extent. 
By connecting each radical structure sequence in the label, we get the sequence modeling label.

%for each tree in the forest, we use the linear radical structure sequence~\cite{fudanvi} by traversing the tree in preorder.
%This sequence retains the hierarchical structure information of Chinese character components to a certain extent. By connecting each radical structure sequence in label, we get the sequence modeling label.

The ARB prediction is supervised with the ARB loss $L_{arb}$, which is a weighted cross-entropy loss of each element.
\begin{equation}
L_{arb}=\sum_{i}^{\variantof{l}{rad}}w_{rad_{(i)}}*logP(r^{*}_{(i)}),
\end{equation}
where $r^{*}_{i}$ is the ground truth of the $i$-th radical, $L$ is the total radical length of \textbf{all} characters in the sample.

The radical structure sequence contains the component and structural information of the label, so this modeling method implements the introduction of hierarchical information and effectively improves the vision model performance.
\subsubsection{Naive Weighting}
We first use a naive way to set equal weights to radicals in each character, i.e, $\mathbf{w}_{rad}=\mathbf{w}_{naive}= \mathbf{1}.$
Albeit the Naive method demonstrates some extent of performance improvement, it treats all components as equal importance, which may lead to over-focusing on minor details.



\subsubsection{TreeED enhanced Weighting}

In sequence modeling, the structural information is implicit, we want to make it more explicit. 
%we want to better model the hierarchical structure of radicals. 
%So we propose to use Tree-edit Distance to calculate the difference between two radial trees. Based on it, 
So we propose TreeED enhanced Weighting method to explicitly strengthen the structural information of label representation.


We add the TreeED weight(\FigTreeEDWeight{}) to the naive weight as a regularization term and get the final radical weight.
\begin{equation}
    w_{radical}= w_{naive} + \lambda_{treeED}w_{treeED}
    %w_{radical}= \frac{{}w_{soft} + \lambda_{ted}w_{ted}}{2}
    %w_{radical}= (1-\lambda{})w_{soft} +  \lambda{}w_{ted},
\end{equation}
where $\lambda_{treeED}$ is set to 1.
This method enhanced the structural information in loss explicitly, which shows better performance on the vision model than the Naive method.


\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/framework3.png}
  \caption{The Structure Aware Network (SAN). The orange square frame is the ARB-TreeED and the blue square frame is the base network. The gradient flow of the ARB-TreeED and the VM decoder influence the feature extractor together.  }
  \label{fig:framewoek}
\end{figure}
\subsection{Structural Aware Network} 
Implementation-wise, we adopt the SOTA ABINet~\cite{ABINet} as the base method, applying ARB yields a novel two branches learning network, which replaces the original Vision Model. The feature is divided into two branches, one is passed into the VM decoder, decoded by characters, and the other is passed into ARB, decoded by radical.
%We combine the module with the SOTA ABINet to demonstrate the efficacy of the proposed ARB module. ARB is added behind the feature extractor. The feature is divided into two branches, one is passed into the VM decoder, decoded by characters, and the other is passed into ARB, decoded by radical.
The training gradient flow by two branches is superimposed and updates the weight of the feature extractor together, which allows the radical level prediction model to supplement and refine the visual feature extraction of the character prediction model in the training process.
%allowing them to update the weight of the feature extractor together.
we define the loss as follows
\begin{equation}
    L_{overall}=L_{base}+L_{arb},
\end{equation}
where $L_{base}$ is the loss of base model, which is the loss from ABINet in this work, i.e.,
\begin{equation}
    L_{base}=L_{vm}+L_{lm}.
\end{equation}

Both the character prediction branch and radical structure prediction branch affect the feature extraction. For fairness, we give them the same weight of influence on visual feature extraction, to ensure that the performance of both parties is fully reflected.

%\begin{figure}[t]	
%    \begin{minipage}[b]{1\linewidth}
%       \centering       
%        \includegraphics[height=2.3cm,width=12cm]{figures/ExampleResult2.png}   
%        \caption{Successful recognition examples using ARB. The two pictures on the left are complex character examples. The two pictures on the right are long-tailed character examples. Text strings are ABINet prediction and ARB-TreeED prediction}
%    \end{minipage}
%    \vspace{-7mm}
%\end{figure}


\begin{figure}[t]	
\centering
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2cm,width=3cm]{figures/result-complex1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Complex]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2cm,width=3cm]{figures/result-complex2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2cm,width=3cm]{figures/result-tail1.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
    \subfigure[Long-tailed]
    {
        \begin{minipage}[t]{0.22\linewidth}
            \centering          %子图居中
            \includegraphics[height=2cm,width=3cm]{figures/result-tail2.png}   
            %\caption{Radical Tree}
        \end{minipage}
    }
\caption{Successful recognition examples using ARB. (a) (b) are complex character examples. (c) (d) are long-tailed character examples. Text strings are ABINet prediction and ARB-TreeED prediction}
%\vspace{-3mm}
\end{figure}



==> ourmethod_intro_v1.tex <==
In this section, we first introduce how to model the label in our work and introduce using Tree-Edit Distance to measure the similarity of two radical trees. Then based on the label modeling method, we propose the Auxiliary Radical Branch and propose two loss design methods to better reflect the structural representation. At last, we integrate the proposed model into a base recognition network and demonstrate its efficacy.
